Visual explanations for polyp detection: How medical doctors assess intrinsic versus extrinsic explanations

Deep learning has in recent years achieved immense success in all areas of computer vision and has the potential of assisting medical doctors in analyzing visual content for disease and other abnormalities. However, the current state of deep learning is very much a black box, making medical professionals highly skeptical about integrating these methods into clinical practice. Several methods have been proposed in order to shine some light onto these black boxes, but there is no consensus on the opinion of the medical doctors that will consume these explanations. This paper presents a study asking medical doctors about their opinion of current state-of-the-art explainable artificial intelligence methods when applied to a gastrointestinal disease detection use case. We compare two different categories of explanation methods, intrinsic and extrinsic, and gauge their opinion of the current value of these explanations. The results indicate that intrinsic explanations are preferred and that explanation.

==> Artificial Intelligence in Medicine - visual explanations polyps/figures/Figure_Case_Examples.tex <==
{

\newcommand{\figurewidth}{0.19\textwidth}

\begin{figure}%[ht!] 
  \centering
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/0b4f0370-b25b-4e6a-a7ac-b09097bfecc3.jpg}
         \caption{}
         \label{figure:user-study-cases-0b4f0370-b25b-4e6a-a7ac-b09097bfecc3-image}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/4_endocv2021_positive_34.jpg}
         \caption{}
         \label{figure:user-study-cases-4_endocv2021_positive_34-image}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/9a48d2e8-12a5-43d6-b20f-1dc7852b4443.jpg}
         \caption{}
         \label{figure:user-study-cases-1dc7852b4443-image}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/14_endocv2021_positive_902.jpg}
         \caption{}
         \label{figure:user-study-cases-14_endocv2021_positive_902-image}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/33fa6aa7-fff7-4bb2-8bd5-2f19c3270595.jpg}
         \caption{}
         \label{figure:user-study-cases-2f19c3270595-image}
     \end{subfigure}
     
     
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/0b4f0370-b25b-4e6a-a7ac-b09097bfecc3-a.png}
         \caption{}
         \label{figure:user-study-cases-b09097bfecc3-a}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/4_endocv2021_positive_34-a.png}
         \caption{}
         \label{figure:user-study-cases-4_endocv2021_positive_34-a}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/9a48d2e8-12a5-43d6-b20f-1dc7852b4443-a.png}
         \caption{}
         \label{figure:user-study-cases-1dc7852b4443-a}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/14_endocv2021_positive_902-a.png}
         \caption{}
         \label{figure:user-study-cases-14_endocv2021_positive_902-a}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/33fa6aa7-fff7-4bb2-8bd5-2f19c3270595-a.png}
         \caption{}
         \label{figure:user-study-cases-2f19c3270595-a}
     \end{subfigure}
     
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/0b4f0370-b25b-4e6a-a7ac-b09097bfecc3-b.png}
         \caption{}
         \label{figure:user-study-cases-b09097bfecc3-b}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/4_endocv2021_positive_34-b.png}
         \caption{}
         \label{figure:user-study-cases-4_endocv2021_positive_34-b}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/9a48d2e8-12a5-43d6-b20f-1dc7852b4443-b.png}
         \caption{}
         \label{figure:user-study-cases-1dc7852b4443-b}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/14_endocv2021_positive_902-b.png}
         \caption{}
         \label{figure:user-study-cases-14_endocv2021_positive_902-b}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/cases/33fa6aa7-fff7-4bb2-8bd5-2f19c3270595-b.png}
         \caption{}
         \label{figure:user-study-cases-2f19c3270595-b}
     \end{subfigure}
     \caption{Five cases taken from the survey presented to each participant. The top row shows the image that was passed through the model to generate a prediction. The second row shows the intrinsic explanation method used to explain the prediction. The last row shows the extrinsic explanation method used to explain the prediction.}\label{figure:case_examples}
\end{figure}

}

==> Artificial Intelligence in Medicine - visual explanations polyps/figures/Figure_Histogram_Multiple_Choice_Questions.tex <==
{

\newcommand{\figurewidth}{0.33\textwidth}

\begin{figure}[ht!]
  \centering
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Histogram_Before_or_After_Procedure.png}
         \caption{}
         \label{figure:histogram-before-after}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Histogram_Explanation_or_Not.png}
         \caption{}
         \label{figure:histogram-explanation-or-not}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Histogram_Most_Useful_Clinical_Practice.png}
         \caption{}
         \label{figure:histogram-most-useful}
     \end{subfigure}
     \caption{The responses collected from the multiple-choice questions asked in the survey.}
\end{figure}

}

==> Artificial Intelligence in Medicine - visual explanations polyps/figures/Figure_Participant_Statistics.tex <==
{

\newcommand{\figurewidth}{0.33\textwidth}

\begin{figure}%[ht!]
  \centering
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/plots/Histogram_Active_Years.png}
         \caption{Number of active years in the medical field.}
         \label{figure:plot-active-years}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/plots/Histogram_Degree.png}
         \caption{The degree(s) obtained by the participants.}
         \label{figure:plot-degree}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[height=\textwidth, width=\textwidth]{images/plots/Histogram_Country.png}
         \caption{The country that the participant comes from.}
         \label{figure:plot-country}
     \end{subfigure}
     \caption{Plots presenting some statistics about the participants included in the study.}\label{figure:participant-statistics}
\end{figure}

}

==> Artificial Intelligence in Medicine - visual explanations polyps/figures/Figure_Violin_Likert_Years_Active.tex <==
{

\newcommand{\figurewidth}{0.33\textwidth}

\begin{figure}%[ht!]
  \centering
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_A_Trust.png}
         \caption{}
         \label{subfigure:trust-a}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_B_Trust.png}
         \caption{}
         \label{subfigure:trust-b}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_A_Understanding.png}
         \caption{}
         \label{subfigure:understanding-a}
     \end{subfigure}
     
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_B_Understanding.png}
         \caption{}
         \label{subfigure:understanding-b}
     \end{subfigure}
      \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_A_Spatial.png}
         \caption{}
         \label{subfigure:spatial-a}
     \end{subfigure}
          \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_B_Spatial.png}
         \caption{}
         \label{subfigure:spatial-b}
     \end{subfigure}
     
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_A_Colors.png}
         \caption{}
         \label{subfigure:colors-a}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_B_Colors.png}
         \caption{}
         \label{subfigure:colors-b}
     \end{subfigure}
     \begin{subfigure}[b]{\figurewidth}
         \centering
         \includegraphics[width=\textwidth]{images/plots/Violin_Experience_Importance.png}
         \caption{}
         \label{subfigure:importance}
     \end{subfigure}
     \caption{A collection of violin plots that presents an overview of the responses collected from the Likert questions. The answers are grouped by the number of years the person has been active in the medical field.}\label{figure:user-study-likert-violin-plots-experience}
\end{figure}

}

==> Artificial Intelligence in Medicine - visual explanations polyps/glossary.tex <==
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{gi}{GI}{gastrointestinal}
\newacronym{ml}{ML}{machine learning}
\newacronym{cnn}{CNN}{machine learning}
\newacronym{xai}{XAI}{explainable artificial intelligence}
\newacronym{shap}{SHAP}{SHapley Additive exPlanations}
\newacronym{gradcam}{GradCAM}{Gradient-weighted Class Activation Mapping}
\newacronym{lime}{LIME}{Local Interpretable Model-Agnostic Explanations}

==> Artificial Intelligence in Medicine - visual explanations polyps/tables/feedback_form_questions.tex <==
\newcommand{\lastcolumnwidth}[0]{7cm}

\begin{table*}%[ht!]
\small
\centering
\caption{The questions that were asked to the participants in the final feedback form. Please note that \textit{Explanation A} refers to the intrinsic explanation and \textit{Explanation B} is the extrinsic explanation.}
\label{table:feedback-form-questions}

\begin{tabular}{l l}

\toprule
Type & Question \\ 
\midrule
\multirow{9}{*}{Likert scale (1-10)} & Explanation (A) increased my understanding of the result. \\
& Explanation (B) increased my understanding of the result. \\
& Explanation (A) increased my trust in the AI model. \\ 
& Explanation (B) increased my trust in the AI model. \\ 
& I found the colors used to visualize explanation (A) to be appropriate. \\ 
& I found the colors used to visualize explanation (B) to be appropriate. \\ 
& Explanation (A) frequently highlighted the correct area in the image. \\
& Explanation (B) frequently highlighted the correct area in the image. \\
& It is important that an explanation accompanies a prediction. \\
\midrule
\multirow{3}{*}{Multiple choice} & Do you prefer to have an explanation, or would you rather only know the prediction? \\
& Which type of explanation would be useful in clinical practice? \\
& Would you prefer that explanations for the predictions be shown during or after the procedure? \\ 
\midrule
\multirow{2}{*}{Free form} & What do you think of explanation method (A)? \\
& What do you think of explanation method (B)? \\
\bottomrule

% Q12: Do you prefer to have an explanation, or would you rather only know the prediction?
% Options: 
% - I prefer the prediction, with an explanation 
% - I prefer the prediction, without an explanation
% Comments (optional)

% Q13: In your opinion, which type of explanation would be useful in clinical practice?
% Options:
% - (A) Intrinsic 
% - (B) Dataset based 
% - Either (A) or (B) 
% - (A) and (B) together 
% - Neither (A) nor (B)

% Q14:Assuming that an AI model is reporting pathological findings live during a colonoscopy procedure, would you prefer that explanations for the predictions be shown during or after the procedure?
% Options:
% - Only during 
% - Only after 
% - Both during and after 
% - Neither during nor after\
% Comments (optional)

\end{tabular}
\end{table*}


==> Artificial Intelligence in Medicine - visual explanations polyps/tables/intraclass_correlation_coefficient.tex <==
\begin{table}
    \centering
    \caption{}\label{tab:intraclass_correlation_coefficient}
    \begin{tabular}{c c c c c c c c c}
         & & \multicolumn{2}{c}{95\% Confidence Interval} &  & \multicolumn{4}{c}{F Test with True Value 0} \\ \cmidrule{3-4} \cmidrule{6-9}
         & Interclass Correlation & Lower Bound & Upper Bound &  & Value & df1 & df2 & Sig \\
        \midrule
            Single Measures &  $0.067$ &  $0.023$ &  $0.220$ & &  $4.852$ & $9$ & $477$ & < $0.000$ \\
            Average Measures &  $0.794$ &  $0.559$ &  $0.938$ & &  $4.852$ & $9$ & $477$ & < $0.000$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> Artificial Intelligence in Medicine - visual explanations polyps/tables/overall_agreement.tex <==
\begin{table}
    \centering
    \caption{}\label{tab:overall_agreement}
    \begin{tabular}{c c c c c c c c}
         & & \multicolumn{3}{c}{Asymptotic}&  & \multicolumn{2}{c}{Asymptotic 95\% Confidence Interval} \\ \cmidrule{3-5} \cmidrule{7-8}
         & Kappa & Standard Error & z & Sig & & Lower Bound & Upper Bound \\
        \midrule
            Overall Agreement & $0.049$ & $0.008$ & $5.878$ & $<.001$ & & $0.033$ & $0.066$ \\
        \bottomrule
    \end{tabular}
\end{table}
